Vertex Deletion on $H$-Induced-Minor-Free Graphs: Subexponential FPT Algorithms and Approximation Schemes

We study vertex-deletion problems on string graphs and, more generally, on graphs excluding a fixed graph as an induced minor. For every fixed graph $H$, fixed nonnegative integer $t$, and fixed monadic second-order formula $\phi$, we consider the problem of finding a minimum-cardinality set $S$ such that $G-S$ has treewidth at most $t$ and satisfies $\phi$. This captures classic problems such as Vertex Cover, Feedback Vertex Set, and deletion to graphs of any fixed bounded treewidth. We give an algorithm with running time $2^{k^{2/3} \log^{O(1)} k}n^{O(1)}$ on $H$-induced-minor-free graphs, where $k$ is the optimum deletion-set size. This resolves in the affirmative the open problem highlighted by Bonnet and Rz\k{a}\.{z}ewski [Algorithmica 2019] and Berthe, Bougeret, Gon\c{c}alves, and Raymond [ICALP 2025] regarding the existence of a subexponential parameterized algorithm for Feedback Vertex Set on string graphs. Our algorithm significantly improves over existing parameterized algorithms for more restricted classes of problems on more restricted classes of graphs. When the property defined by $\phi$ is hereditary, we also obtain a quasi-polynomial time approximation scheme, namely an algorithm that produces a $(1+\varepsilon)$-approximate solution in quasi-polynomial time. Both the sub-exponential algorithm and the quasi-polynomial time approximation scheme build on the same new structural and algorithmic insights.

==> Quasipolytime.tex <==
Fix a graph $H$ and an integer $t\geq1$. Let $\mathcal G_H$ denote
 the class of graphs excluding $H$ as an induced minor. For every graph $F$,
 define
\[
 \operatorname{OPT}_t(F)
 =\min\{|S|:S\subseteq V(F),\ \operatorname{tw}(F-S)\leq t\}.
\]
A set $S$ satisfying $\operatorname{tw}(F-S)\leq t$ is a
\emph{treewidth-$t$ modulator}. The problem considered throughout
this note is to find a minimum such set.

We prove a total-cost guarantee: a structural deletion set $X$
leaves bounded treewidth and can be completed to a near-optimal
solution. The algorithm returns a single pair of deletion sets.
Its recursive calls return one minimum cost and an attaining pair.

\paragraph{Algorithmic inputs.}
The main input is the following theorem from the manuscript.
\begin{inputtheorem}
For fixed $H$, given $F\in\mathcal G_H$ and parameters $b,d,t$, an
algorithm running in $b^{O(t^2b/d)}|V(F)|^{O(1)}$ time outputs at most
$b^{O(t^2b/d)}$ sets $A\subseteq V(F)$, each satisfying
$\operatorname{tw}(F-A)\leq C_{H,t}\sqrt{bd}$. For every treewidth-$t$
modulator $S$ of size at most $b$, at least one output satisfies
$A\subseteq S$.
\end{inputtheorem}

We also use the following two routines from the manuscript.
First, the modulator approximation of Lemma~2.8 finds, in polynomial
time for fixed $t$, a treewidth-$t$ modulator $W_0$ of size at most
$a_t\operatorname{OPT}_t(G)$, for a constant $a_t\geq1$ depending only
on $t$; see~\cite{DBLP:conf/soda/GuptaLLM019}.
Second, the bounded-treewidth deletion algorithm of Lemma~4.1,
specialized to treewidth deletion, finds an exact minimum
 treewidth-$t$ modulator on a graph of treewidth at most $B$ in time
$g(t,B)n^{O(1)}$. We use this second routine only when $B$ is bounded
by a function of $H,t,\varepsilon$.

\setcounter{section}{1}
\setcounter{lemma}{1}
\begin{restatable}{theorem}{qptas}\label{thm:qptas}
Fix a graph $H$ and an integer $t\geq1$. Assuming the input branching
theorem, Treewidth-$t$ Deletion on $\mathcal G_H$ admits a
quasipolynomial-time approximation scheme. More precisely, for every
$0<\varepsilon\leq1$, there is an algorithm that, given $G\in\mathcal G_H$,
returns a treewidth-$t$ modulator $D$ satisfying
\[
 |D|\leq(1+\varepsilon)\operatorname{OPT}_t(G).
\]
Writing $k=\operatorname{OPT}_t(G)$ and $n=|V(G)|$, its running time is
\[
 f(H,t,\varepsilon)\,
 2^{O_{H,t}(\varepsilon^{-2}\log^{10}(k+2))}\,n^{O(1)}.
\]
The algorithm does not need to know $k$.
\end{restatable}

\setcounter{section}{4}
\setcounter{lemma}{1}
\setcounter{algorithm}{1}
\subsection{A structural deletion set with a near-optimal completion}
\providecommand{\QPOpt}{\operatorname{OPT}_t}
\providecommand{\QPTw}{\operatorname{tw}}
All logarithms have base two. Write $L(q)=\log(q+2)$.
Constants with subscript $H,t$ may depend on $H,t$, but not on
$\varepsilon$ or the input size.

\begin{lemma}[Local branching and separation]
\label{lem:qp-local}
There are constants $c_1,c_2>0$, depending only on $H,t$, with the
following property. Let $0<\delta\leq 1/2$. For every sufficiently large
$q$, where the threshold depends only on $H,t,\delta$, given a graph
$F\in\mathcal G_H$ and a set $W\subseteq V(F)$ of size $q$, one can
compute a family $\mathcal A$ and, for each $A\in\mathcal A$, a set
$Z_A\subseteq V(F)\setminus A$ and two vertex-disjoint induced subgraphs
$F_{A,1},F_{A,2}$ such that:
\begin{enumerate}[(i)]
\item $F-(A\cup Z_A)$ is the disjoint union of $F_{A,1},F_{A,2}$;
\item $|W\cap V(F_{A,j})|\leq 2q/3$ for $j\in\{1,2\}$;
\item $|Z_A|\leq c_1q/L(q)^2$;
\item if $S\subseteq V(F)$ satisfies $\QPTw(F-S)\leq t$ and
      $|S|\leq q/\delta$, then some $A\in\mathcal A$ satisfies $A\subseteq S$.
\end{enumerate}
The family size is at most $2^{c_2\delta^{-2}L(q)^9}$ and the running
time is $2^{c_2\delta^{-2}L(q)^9}|V(F)|^{O(1)}$.
\end{lemma}

\begin{proof}
Set
\[
 b=\left\lceil q/\delta\right\rceil,
 \qquad d=\left\lceil\delta q/L(q)^8\right\rceil.
\]
Choose the threshold large enough that, for all $q$ above it,
$q\geq 1/\delta$ and $\delta q/L(q)^8\geq 1$.
Then
\[
 b\leq 2q/\delta,\qquad
 \frac{\delta q}{L(q)^8}\leq d\leq\frac{2\delta q}{L(q)^8},\qquad
 \frac bd\leq 2\delta^{-2}L(q)^8.
\]
Apply \QPBranchRef\ to $F$ with parameters $b,d,t$. Its family
$\mathcal A$ has size $b^{O(t^2b/d)}$. Since
$\log(b+2)=O(L(q))$, this is at most
$2^{c_2\delta^{-2}L(q)^9}$ after increasing $c_2$.
Its containment guarantee gives (iv), and for each output $A$,
\[
 \QPTw(F-A)\leq C_{H,t}\sqrt{bd}
                    \leq 2C_{H,t}\frac q{L(q)^4}.
\]

The polynomial-time treewidth approximation of Feige, Hajiaghayi,
and Lee~\cite{FHL2008} computes a decomposition of width
$O((w+1)\sqrt{\log(w+2)})$ when the treewidth is $w$.
Consequently, after increasing the threshold and the constants,
we obtain a decomposition of $F-A$ of width at most
$C'_{H,t}q/L(q)^3$. We only need the weaker bound with $L(q)^2$
in the denominator.

Give weight one to every vertex of $W\setminus A$ and zero to
every other vertex. A weighted balanced bag of this decomposition
gives a set $Z_A$ such that every component of $F-(A\cup Z_A)$
contains at most $|W\setminus A|/2\leq q/2$ marked vertices.
The balanced bag can be found by assigning each marked vertex to
one bag containing it and finding a weighted centroid of the
decomposition tree. The extra one in the bag size is absorbed by
$c_1q/L(q)^2$ for sufficiently large $q$. If $F-A$ is empty, take
$Z_A=\emptyset$ and both child graphs empty.

To obtain two child graphs, consider the weights of the components
of $F-(A\cup Z_A)$. Their total is at most $q$, and each weight
is at most $q/2$. If one component has weight in $[q/3,2q/3]$,
put it in the first group and all others in the second group.
Otherwise, all component weights are less than $q/3$. If their
total is at least $q/3$, accumulate components until the weight
first reaches $q/3$; the resulting weight is less than $2q/3$,
and the remaining weight is at most $2q/3$. If the total is less
than $q/3$, put all components in one group. Components of weight
zero can be assigned arbitrarily. The induced graphs on the two
groups satisfy (i) and (ii). All work beyond the application of
\QPBranchRef\ is polynomial per output set.
\end{proof}

\begin{lemma}[Charging separators]
\label{lem:qp-charge}
Let $T$ be a rooted binary tree. Associate a set $W_v$ with each
node $v$, and write $q_v=|W_v|$. Suppose that the two child sets
are disjoint subsets of their parent set, and every child $u$ of
$v$ satisfies $q_u\leq 2q_v/3$. Let $Q\geq 2$, and suppose every
internal node has $q_v>Q$. Then, for an absolute constant $c_0$,
\[
 \sum_{v\text{ internal}}\frac{q_v}{L(q_v)^2}
       \leq \frac{c_0|W_{\mathrm{root}}|}{L(Q)}.
\]
\end{lemma}

\begin{proof}
Distribute the summand at $v$ equally among the vertices of $W_v$.
Each such vertex receives $1/L(q_v)^2$. For a fixed vertex $x$ of
$W_{\mathrm{root}}$, the nodes containing $x$ form a root-to-node
path, since child sets are disjoint subsets of their parent set.
List the internal nodes on this path in reverse order, starting
with the deepest one. If their weights are $q_0,q_1,\ldots$, then
\[
 q_j\geq (3/2)^j q_0>(3/2)^j Q.
\]
Writing $s=\log Q\geq 1$ and $\gamma=\log(3/2)>0$, the total
charge to $x$ is at most
\[
 \sum_{j\geq 0}\frac1{(s+j\gamma)^2}
 \leq\frac1{s^2}+\int_0^\infty\frac{du}{(s+\gamma u)^2}
 =\frac1{s^2}+\frac1{\gamma s}
 \leq\frac{c_0}{L(Q)}.
\]
The last inequality holds for a suitable absolute constant because
$L(Q)\leq 2\log Q$ for $Q\geq 2$. Summing over all root vertices
proves the result.
\end{proof}

\begin{corollary}[Structural deletion with a near-optimal completion]
\label{cor:qpbranching}
Fix a graph $H$ and an integer $t\geq1$. Assuming the input branching
theorem, for every $0<\varepsilon\leq1$ there is an algorithm that,
given $G\in\mathcal G_H$, computes disjoint sets $X,Y\subseteq V(G)$
satisfying
\begin{enumerate}[(i)]
\item $\QPTw(G-X)\leq B$, where
      $B=B(H,t,\varepsilon)=2^{O_{H,t}(1/\varepsilon)}$;
\item $\QPTw(G-(X\cup Y))\leq t$;
\item $|X|+|Y|\leq(1+\varepsilon)\QPOpt(G)$.
\end{enumerate}
In particular,
\[
 \boxed{|X|+\QPOpt(G-X)\leq(1+\varepsilon)\QPOpt(G).}
\]
With $k=\QPOpt(G)$ and $n=|V(G)|$, the running time is at most
\[
 f(H,t,\varepsilon)\,
 2^{O_{H,t}(\varepsilon^{-2}\log^{10}(k+2))}\,n^{O(1)}.
\]
\end{corollary}

\begin{proof}
We describe the structural choices, show that they include one of
sufficiently small completion cost, and then give a scalar recurrence
that finds the best completion cost among all these choices.

\paragraph{Initial modulator and threshold.}
By \QPModRef, compute a treewidth-$t$ modulator $W_0$ such that
\[
 |W_0|\leq a_t\,\operatorname{OPT}_t(G)\leq a_t k,
 \qquad \QPTw(G-W_0)\leq t,
\]
where $\operatorname{OPT}_t$ denotes deletion to treewidth at most
$t$, and $a_t\geq 1$ is a
constant depending only on $t$. Small fixed values of $t$ are
absorbed in $a_t$.
Set $\delta=\varepsilon/2$. Let $c_1$ be the constant from
Lemma~\ref{lem:qp-local}, and let $c_0$ be the constant from
Lemma~\ref{lem:qp-charge}. Choose an integer $Q\geq 2$ so that
Lemma~\ref{lem:qp-local} applies to every $q>Q$ and
\begin{equation}
 \frac{c_0c_1a_t}{L(Q)}\leq\frac\varepsilon2.
 \label{eq:qp-threshold}
\end{equation}
We may choose $Q=\lceil 2^{D_{H,t}/\varepsilon}\rceil$ for a
sufficiently large constant $D_{H,t}$. Indeed, this choice satisfies
\eqref{eq:qp-threshold}, $Q\geq 1/\delta$, and
$\delta q/L(q)^8\geq 1$ for every $q>Q$, after increasing
$D_{H,t}$. The remaining threshold requirements in
Lemma~\ref{lem:qp-local} depend only on $H,t$.
Put $B=t+Q$.

Every recursive instance is a pair $(F,W)$, where $F$ is an induced
subgraph of $G$ and $W=W_0\cap V(F)$. In particular,
\begin{equation}
 \QPTw(F-W)\leq t.
 \label{eq:qp-invariant}
\end{equation}
The root instance is $(G,W_0)$.

\paragraph{Structural choices.}
At an instance $(F,W)$, put $q=|W|$.
If $q\leq Q$, stop with structural deletion set $\emptyset$ and
terminal graph $F$. By \eqref{eq:qp-invariant},
\[
 \QPTw(F)\leq t+q\leq B.
\]
For example, a width-$t$ decomposition of $F-W$ becomes a
width-$(t+q)$ decomposition after adding $W$ to every bag; if
$F-W$ is empty, use the single bag $W$.

If $q>Q$, include the following alternatives:
\begin{enumerate}[(a)]
\item Delete $W$ structurally and stop with terminal graph $F-W$.
      This terminal graph has treewidth at most $t$.
\item Apply Lemma~\ref{lem:qp-local}. For each $A\in\mathcal A$,
      delete $A\cup Z_A$ structurally, and recurse on both
      $(F_{A,1},W_0\cap V(F_{A,1}))$ and
      $(F_{A,2},W_0\cap V(F_{A,2}))$.
\end{enumerate}
Each recursive child has at most $2q/3$ marked vertices. Hence
the recursion terminates. For any complete choice of alternatives,
let $X$ be the union of all structural deletions. The graph $G-X$
is a disjoint union of terminal graphs, each of treewidth at most
$B$. Therefore every represented structural set satisfies
\begin{equation}
 \QPTw(G-X)\leq B.
 \label{eq:qp-all-width}
\end{equation}
The recursion is an implicit representation: we do not form the
Cartesian products of the families represented by its two children.

\paragraph{A good construction for a fixed optimum.}
Fix an optimum treewidth-$t$ deletion set $S^\star$ of $G$; thus
$|S^\star|=k$. At a recursive instance, let
$s_F=|S^\star\cap V(F)|$. The restriction
$S^\star\cap V(F)$ is a treewidth-$t$ modulator of $F$.
Select a complete structural construction by the following rule,
used only in the analysis:
\begin{itemize}
\item If $q\leq Q$, stop without a structural deletion.
\item If $q>Q$ and $s_F>q/\delta$, select alternative (a).
\item Otherwise, $s_F\leq q/\delta$. By
      Lemma~\ref{lem:qp-local}(iv), some $A\in\mathcal A$ satisfies
      $A\subseteq S^\star\cap V(F)$. Select this $A$ in alternative
      (b), and continue in both children.
\end{itemize}
The algorithm does not know $s_F$ or $S^\star$; it considers all
the alternatives needed by this rule.

Let $X^\star$ be the resulting structural deletion set. At every
selected split, $A\subseteq S^\star$, so these sets add no vertices
to $X^\star\setminus S^\star$. At a selected terminal alternative
(a),
\[
 |W\setminus S^\star|\leq q<\delta s_F.
\]
The graphs at distinct such terminal nodes have disjoint vertex
sets. Thus the total contribution of these alternatives is at most
\begin{equation}
 \delta\sum_F s_F\leq\delta k=\frac{\varepsilon k}{2}.
 \label{eq:qp-terminal-loss}
\end{equation}

Apply Lemma~\ref{lem:qp-charge} to the selected structural recursion
tree, with marked sets $W_0\cap V(F)$. Every internal node has
$q>Q$, its child sets are disjoint subsets of its marked set, and
each child has weight at most $2q/3$. Consequently,
\begin{align}
 \sum_{F\text{ split}}|Z_F|
 &\leq c_1\sum_{F\text{ split}}\frac{|W_0\cap V(F)|}
                                      {L(|W_0\cap V(F)|)^2}\notag\\
 &\leq\frac{c_0c_1|W_0|}{L(Q)}
 \leq\frac{c_0c_1a_t k}{L(Q)}
 \leq\frac{\varepsilon k}{2}.
 \label{eq:qp-separator-loss}
\end{align}
Together, \eqref{eq:qp-terminal-loss} and
\eqref{eq:qp-separator-loss} imply
\begin{equation}
 |X^\star\setminus S^\star|\leq\varepsilon k.
 \label{eq:qp-witness-loss}
\end{equation}
The graph
$G-(X^\star\cup S^\star)$ is an induced subgraph of $G-S^\star$.
It has treewidth at most $t$, since treewidth does not increase
under vertex deletion.
Thus $Y^\star=S^\star\setminus X^\star$ is a feasible completion,
and
\begin{equation}
 |X^\star|+|Y^\star|
 =|S^\star|+|X^\star\setminus S^\star|
 \leq(1+\varepsilon)k.
 \label{eq:qp-witness-cost}
\end{equation}

\paragraph{Additivity of the completion cost.}
If $J_1,J_2$ are vertex-disjoint and there are no edges between them, then
\begin{equation}
 \QPOpt(J_1\mathbin{\dot\cup}J_2)=\QPOpt(J_1)+\QPOpt(J_2).
 \label{eq:tw-additive}
\end{equation}
Indeed, restricting any feasible deletion set to a component gives
feasible deletion sets in the two graphs. Conversely, the union of
minimum deletion sets is feasible, because the treewidth of a disjoint
union is the maximum of the treewidths of its components.

\paragraph{The scalar recurrence.}
At each instance $(F,W)$, return a triple $(c,X,Y)$, where $c=|X|+|Y|$,
the sets $X,Y$ are disjoint, and
\[
 \QPTw(F-X)\leq B,
 \qquad
 \QPTw(F-(X\cup Y))\leq t.
\]
The scalar $c$ is minimized over the structural choices represented
by the recursion and their exact completion costs.
Write $\mathsf C(F,W)$ for this minimum cost.

If $q=|W|\leq Q$, solve Treewidth-$t$ Deletion exactly on $F$.
For a minimum deletion set $D$, return
\[
 (\mathsf C(F,W),X,Y)=(|D|,\emptyset,D).
\]
If $q>Q$, initialize the answer to $(q,W,\emptyset)$.
This is feasible by \eqref{eq:qp-invariant}. In particular, the
option of deleting $W$ needs no further deletion and no recursive call.
For each candidate $A$ in Lemma~\ref{lem:qp-local}, set
$W_j=W_0\cap V(F_{A,j})$ and recursively obtain
$(\kappa_j,X_j,Y_j)$ from $(F_{A,j},W_j)$ for $j\in\{1,2\}$.
This candidate yields
\begin{align*}
 c_A&=|A|+|Z_A|+\kappa_1+\kappa_2,\\
 X_A&=A\cup Z_A\cup X_1\cup X_2,\\
 Y_A&=Y_1\cup Y_2.
\end{align*}
Keep the triple of smallest cost among the initial answer and all
these candidates. Equivalently,
\begin{equation}
\begin{split}
 \mathsf C(F,W)=\min\bigl\{q,\ \min_{A\in\mathcal A}\bigl(
 |A|+|Z_A| &+\mathsf C(F_{A,1},W_1)\\
            &+\mathsf C(F_{A,2},W_2)\bigr)\bigr\}
 \qquad(q>Q).
\end{split}
\label{eq:tw-recurrence}
\end{equation}
An empty minimum over $\mathcal A$ is interpreted as $+\infty$;
the option of deleting $W$ is always available.

\begin{algorithm}[t]
\caption{\textsc{Solve}$(F,W)$ for Treewidth-$t$ Deletion}
\label{alg-quasibranch}
\small
\noindent\textbf{Input:} $W=W_0\cap V(F)$; fixed $\delta,Q,t$.
\begin{enumerate}
\item Set $q\gets|W|$.
\item If $q\leq Q$, compute a minimum treewidth-$t$ modulator $D$ of
      $F$ and return $(|D|,\emptyset,D)$.
\item Initialize $(c,X,Y)\gets(q,W,\emptyset)$.
\item Compute $\mathcal A$ and the associated separators and child
      graphs using Lemma~\ref{lem:qp-local}.
\item For every $A\in\mathcal A$:
 \begin{enumerate}[(a)]
 \item For $j\in\{1,2\}$, obtain
       $(\kappa_j,X_j,Y_j)\gets\textsc{Solve}(F_{A,j},W_0\cap V(F_{A,j}))$.
 \item Set $c_A\gets|A|+|Z_A|+\kappa_1+\kappa_2$.
 \item If $c_A<c$, replace $(c,X,Y)$ by
       \[
       (c_A,\ A\cup Z_A\cup X_1\cup X_2,\ Y_1\cup Y_2).
       \]
 \end{enumerate}
\item Return $(c,X,Y)$.
\end{enumerate}
\end{algorithm}

\paragraph{Correctness of the recurrence.}
We prove by induction over recursive calls that the returned triple
is feasible and has minimum completion cost over all represented
structural choices.
At a small-$q$ leaf the only structural choice is $X=\emptyset$,
and the exact computation returns its optimum completion.
At an internal node, deleting $W$ has cost exactly $q$, since
$\QPOpt(F-W)=0$.

For a split candidate $A$, all of
$A,Z_A,V(F_{A,1}),V(F_{A,2})$ are pairwise disjoint.
There is therefore no double counting in $c_A$.
Moreover, there are no edges between the child graphs. Applying
\eqref{eq:tw-additive} after their structural deletions shows that
the minimum completion cost for this split is exactly the sum in
\eqref{eq:tw-recurrence}. Each child can be optimized independently.
The union of the resulting witnesses satisfies both treewidth
bounds, because each remaining graph is a disjoint union of the
corresponding child graphs. Taking the minimum over the stop option
and all split candidates proves the induction step.

In particular, for the root pair $(X,Y)$ returned by the algorithm,
\[
 |X|+|Y|=\min_{X'\text{ represented}}
             \bigl(|X'|+\QPOpt(G-X')\bigr).
\]
The analytical construction $X^\star$ above is represented, and
$S^\star\setminus X^\star$ is a feasible completion of it. Therefore,
by \eqref{eq:qp-witness-cost},
\begin{align*}
 |X|+|Y|
 &\leq |X^\star|+\QPOpt(G-X^\star)\\
 &\leq |X^\star|+|S^\star\setminus X^\star|\\
 &\leq(1+\varepsilon)k.
\end{align*}
This proves (iii); feasibility of the stored witnesses proves (i)
and (ii). The displayed total-cost guarantee in the corollary follows
also from $\QPOpt(G-X)\leq|Y|$.
The algorithm need not return the analytical witness $X^\star$:
it returns a structural set of no greater total completion cost.

\paragraph{Running time.}
Let $q_0=|W_0|\leq a_tk$. Each recursive child has at most $2/3$ of
its parent's number of marked vertices. The recursion depth is
therefore $O(\log(q_0+2))$; when $q_0=0$, it consists only of the root.
At a node with $q>Q$, the number of split candidates is at most
\[
 R(q)=2^{c_2\delta^{-2}L(q)^9},
\]
where $c_2$ is the constant from Lemma~\ref{lem:qp-local}.
Each candidate gives two recursive calls, whereas the option of
deleting $W$ gives none. The total number of calls is at most
\[
 (1+2R(q_0))^{O(\log(q_0+2))}
 =2^{O_{H,t}(\delta^{-2}\log^{10}(q_0+2))}.
\]
The two child calls are executed separately, and their returned
costs are added. We never enumerate all pairs of their structural
choices. Consequently, the relevant bound counts recursive calls,
not complete combinations of choices throughout the recursion tree.

A small-$q$ terminal graph has treewidth at most $B=t+Q$.
Its exact solution takes $g(t,B)n^{O(1)}$ time using the stated
bounded-treewidth routine. Computing each candidate separator and
its two child graphs takes polynomial time, in addition to the
branching cost in Lemma~\ref{lem:qp-local}. Witness reconstruction
has polynomial overhead per call. Substituting
$\delta=\varepsilon/2$, $q_0\leq a_tk$, and
$B=2^{O_{H,t}(1/\varepsilon)}$ gives
\[
 f(H,t,\varepsilon)\,
 2^{O_{H,t}(\varepsilon^{-2}\log^{10}(k+2))}\,n^{O(1)}.
\]
The initial approximation, all thresholds, and all recursive
parameters can be computed without knowing $k$.
\end{proof}

\qptas*
\begin{proof}
Apply Corollary~\ref{cor:qpbranching} and return $D=X\cup Y$.
The set $D$ is a treewidth-$t$ modulator, and
$|D|=|X|+|Y|\leq(1+\varepsilon)\QPOpt(G)$.
For fixed $H,t,\varepsilon$, the running time is quasipolynomial
in $n$, because $k\leq n$.
\end{proof}
